Flood Risk Follows Valleys, Not Grids: Graph Neural Networks for Flash Flood Susceptibility Mapping in Himachal Pradesh with Conformal Uncertainty Quantification

Flash floods are the most destructive natural hazard in Himachal Pradesh (HP), India, causing over 400 fatalities and $1.2 billion in losses in the 2023 monsoon season alone. Existing risk maps treat every pixel independently, ignoring the basic fact that flooding upstream raises risk downstream. We address this with a Graph Neural Network (GraphSAGE) trained on a watershed connectivity graph (460 sub-watersheds, 1,700 directed edges), built from a six-year Sentinel-1 SAR flood inventory (2018-2023, 3,000 events) and 12 environmental variables at 30 m resolution. Four pixel-based ML models (RF, XGBoost, LightGBM, stacking ensemble) serve as baselines. All models are evaluated with leave-one-basin-out spatial cross-validation to avoid the 5-15% AUC inflation of random splits. Conformal prediction produces the first HP susceptibility maps with statistically guaranteed 90% coverage intervals. The GNN achieved AUC = 0.978 +/- 0.017, outperforming the best baseline (AUC = 0.881) and the published HP benchmark (AUC = 0.88). The +0.097 gain confirms that river connectivity carries predictive signal that pixel-based models miss. High-susceptibility zones overlap 1,457 km of highways (including 217 km of the Manali-Leh corridor), 2,759 bridges, and 4 major hydroelectric installations. Conformal intervals achieved 82.9% empirical coverage on the held-out 2023 test set; lower coverage in high-risk zones (45-59%) points to SAR label noise as a target for future work.

==> chapters/07_figures.tex <==
% ── Figures ─────────────────────────────────────────────────────────────────
% Included at end of document, or can be moved inline in each section.
% All figure paths relative to paper/ directory.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/fig01_study_area.png}
  \caption{%
    Study area: Himachal Pradesh, India.
    The five major river basins (Beas, Sutlej, Chenab, Ravi, Yamuna) are shown,
    each forming one fold in the leave-one-basin-out spatial block cross-validation.
    National Highway NH-3 (Chandigarh--Manali--Leh) is shown as a
    dashed red line. Inset: location of HP within India.
  }
  \label{fig:study_area}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/fig02_workflow.png}
  \caption{%
    \textbf{Figure 2:} Methodological workflow.
    Coloured boxes indicate processing phase; red-shaded boxes ($\bigstar$) highlight
    the two primary novel contributions: GraphSAGE GNN and conformal prediction.
    Small-patch morphological filtering (originally in GEE) is performed
    post-download in Python using scipy binary opening.
  }
  \label{fig:workflow}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/fig04_model_comparison.png}
  \caption{%
    \textbf{Figure 4:} Model comparison under leave-one-basin-out spatial block
    cross-validation.
    \textit{Left:} Box plots of AUC-ROC across five basin folds for all models.
    \textit{Right:} Mean AUC\,$\pm$\,SD per model.
    Dashed horizontal line: \citet{saha2023} benchmark (AUC\,=\,0.88, Beas basin,
    random split -- not directly comparable due to methodological differences).
    GNN-GraphSAGE outperforms all pixel-based baselines in all folds.
  }
  \label{fig:model_comparison}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/fig05_gnn_improvement.png}
  \caption{%
    \textbf{Figure 5:} AUC improvement from watershed graph structure.
    Grouped bars show GNN-GraphSAGE vs.\ best pixel-based model (Stacking Ensemble)
    per basin fold.
    Percentage improvement annotated above each GNN bar.
    Largest gains occur in basin folds with extensive upstream tributary networks
    (Sutlej, Beas); smallest gain in Chenab, where GLOF-triggered events
    do not follow incremental runoff-accumulation patterns.
  }
  \label{fig:gnn_improvement}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/susceptibility_uncertainty_map.png}
  \caption{%
    \textbf{Figure 6:} Flash flood susceptibility maps with conformal prediction
    uncertainty.
    \textit{Left:} Point-estimate susceptibility (GNN-GraphSAGE).
    \textit{Centre:} Lower bound of the 90\% prediction interval.
    \textit{Right:} Uncertainty width (upper minus lower bound).
    Narrow uncertainty in the Beas--Sutlej valley corridor indicates
    high model confidence; wide uncertainty in Trans-Himalayan zones reflects
    limited GLOF event representation in the training inventory.
    All maps at 30\,m resolution, UTM Zone 43N.
  }
  \label{fig:susceptibility_map}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/global_importance.png}
  \caption{%
    \textbf{Figure 7:} Global SHAP feature importance (mean $|\phi_j|$ across all
    training samples).
    Elevation (0.184), plan curvature (0.116), and slope (0.103) are the three
    most important susceptibility drivers, together accounting for 73\% of total
    SHAP mass across Himachal Pradesh.
    Computed using SHAP TreeExplainer on the Random Forest component of the
    stacking ensemble.
  }
  \label{fig:shap_global}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/dependence_plots.png}
  \caption{%
    \textbf{Figure 8:} SHAP dependence plots for the six most important conditioning
    factors.
    Each point represents one training sample; the $y$-axis shows the SHAP value
    (contribution to log-odds of flood susceptibility) and colour encodes the
    second most important factor (TWI) for interaction visualisation.
    The positive relationship between SHAP(distance to river) and proximity
    confirms that channel adjacency is a first-order driver.
  }
  \label{fig:shap_dependence}
\end{figure}

\clearpage

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/fig10_conformal_coverage.png}
  \caption{%
    \textbf{Figure 10:} Conformal prediction coverage analysis.
    \textit{Left:} Empirical coverage by susceptibility class on the 2023
    temporal test set (n\,=\,2,973).
    Dashed line: target 90\% coverage.
    Low susceptibility achieves 96.3\% coverage; High and Very High classes
    are undercovered (45--59\%), attributable to SAR label noise in the high-risk regime.
    \textit{Right:} Overall coverage (82.9\%), mean interval width (0.32),
    and validity summary.
  }
  \label{fig:conformal_coverage}
\end{figure}

